On Resolving Non-determinism in Choreographies

Choreographies specify multiparty interactions via message passing. A realisation of a choreography is a composition of independent processes that behave as specified by the choreography. Existing relations of correctness/completeness between choreographies and realisations are based on models where choices are non-deterministic. Resolving non-deterministic choices into deterministic choices (e.g., conditional statements) is necessary to correctly characterise the relationship between choreographies and their implementations with concrete programming languages. We introduce a notion of realisability for choreographies - called whole-spectrum implementation - where choices are still non-deterministic in choreographies, but are deterministic in their implementations. Our notion of whole spectrum implementation rules out deterministic implementations of roles that, no matter which context they are placed in, will never follow one of the branches of a non-deterministic choice. We give a type discipline for checking whole-spectrum implementations. As a case study, we analyse the POP protocol under the lens of whole-spectrum implementation.

==> Makefile <==
NOTES = main
t = main
c = "checkpoint"
SOLUT = solutions
LATEX = latexmk -latex="pdflatex --shell-escape"
#MKIDX = makeindex
BIBTEX = bibtex
SUBDIR = .
PDFotp = -sPAPERSIZE=a4
title = hell-lmcs18
host := $(shell hostname -s)
wdir = $(if $(filter em-dell, $(host)), et52@pc1299.mcs.le.ac.uk:/var/cscampus/teaching/resources/CO7205/,/var/cscampus/teaching/resources/CO7205/)
CP = $(if $(filter em-dell, $(host)), scp, cp)
#web = $(if $(filter em-dell, $(host)), et52@pc1299.mcs.le.ac.uk:$(wdir), $(wdir))

all:
	-$(LATEX) $(NOTES).tex
	$(warning **** WARNINGS ****)
	grep Warning $(NOTES).log

bib:
	$(BIBTEX) $(NOTES)

clean:
	find . -name "*~" -exec rm -rf {} \;
	find . -name "*.log" -exec rm -rf {} \;
	find . -name "*.aux" -exec rm -rf {} \;
	find . -name "*.out" -exec rm -rf {} \;
	find . -name "*.synctex.gz" -exec rm -rf {} \;
	find . -name "*.blg" -exec rm -rf {} \;
	find . -name "*.fdb*" -exec rm -rf {} \;
	find . -name "*.fls*" -exec rm -rf {} \;
	find . -name "$(NOTES)*pdf" -exec rm -rf {} \;
	rm -fr auto

e:
	emacs --reverse -T $(title) -mm $(t).tex &

svn:
	svn up
	svn commit -m "$(c)"

